DeepDualMapper: A Gated Fusion Network for Automatic Map Extraction using Aerial Images and Trajectories

Automatic map extraction is of great importance to urban computing and location-based services. Aerial image and GPS trajectory data refer to two different data sources that could be leveraged to generate the map, although they carry different types of information. Most previous works on data fusion between aerial images and data from auxiliary sensors do not fully utilize the information of both modalities and hence suffer from the issue of information loss. We propose a deep convolutional neural network called DeepDualMapper which fuses the aerial image and trajectory data in a more seamless manner to extract the digital map. We design a gated fusion module to explicitly control the information flows from both modalities in a complementary-aware manner. Moreover, we propose a novel densely supervised refinement decoder to generate the prediction in a coarse-to-fine way. Our comprehensive experiments demonstrate that DeepDualMapper can fuse the information of images and trajectories much more effectively than existing approaches, and is able to generate maps with higher accuracy.

==> tab/dataloss_atk.tex <==
\begin{table}
	\scriptsize
	\vspace{-0.2in}
	\caption{\label{tab:dataloss_atk} \textls[-8]{The reported IoU under the test set with information loss attack. Note we do not include the attack in training set.}}
	%\vspace{-0.2in}
	\begin{center}
		\begin{tabular}{c|ccc}
			\hline
			Dataset & Porto & Shanghai & Singapore\\
			%Dataset & \multicolumn{1}{c||}{Porto} & \multicolumn{1}{c||}{Shanghai} & \multicolumn{1}{c}{Singapore}\\
			%\hline
			%Metric & IoU & & IoU & F1-score\\
			\hline
			Early Fusion & 0.500$\pm$0.023 & 0.440$\pm$0.014 & 0.420$\pm$0.016 \\
			Late Fusion & 0.475$\pm$0.011 & 0.407$\pm$0.059 & 0.379$\pm$0.035 \\
			SegNet-RC & 0.546$\pm$0.025 & 0.442$\pm$0.028 & 0.393$\pm$0.026 \\
			FuseNet & 0.463$\pm$0.042 & 0.455$\pm$0.012 & 0.405$\pm$0.039\\
			V-FuseNet & 0.530$\pm$0.028 & 0.432$\pm$0.043 & 0.445$\pm$0.016 \\
			L3Fsn & 0.510$\pm$0.027 & 0.450$\pm$0.011 & 0.391$\pm$0.045\\
			1D decoder & 0.471$\pm$0.043 & 0.455$\pm$0.005 & 0.411$\pm$0.037\\
			TriSeg & 0.462$\pm$0.030 & 0.467$\pm$0.022 & 0.398$\pm$0.024 \\
			\model & \textbf{0.588$\pm$0.019} & \textbf{0.497}$\pm$\textbf{0.023} & \textbf{0.477}$\pm$\textbf{0.030} \\
			\hline
		\end{tabular}
	\end{center}   
	\vspace{-0.2in}
\end{table}


==> tab/overall_eval.tex <==
%
\begin{table*}
	\scriptsize
	%\vspace{-0.3in}
	\caption{\label{tab:overall_eval} The performance of all approaches under three image-trajectory-paired datasets. TC1, KDE and COBWEB are not learning-based approaches thus their results are deterministic.}
	%\vspace{-0.2in}
	\begin{center}
		\begin{tabular}{c|cc||cc||cc}
			\hline
			Dataset & \multicolumn{2}{c||}{Porto} & \multicolumn{2}{c||}{Shanghai} & \multicolumn{2}{c}{Singapore}\\
			\hline
			Metric & IoU & F1-score & IoU & F1-score & IoU & F1-score\\
			\hline
			\multicolumn{7}{c}{\textbf{Trajectory-based Approaches}}\\
			\hline
			TC1 & $0.153 \pm 0.000$ & $0.184 \pm 0.000$ & $0.361 \pm 0.000$ & $0.531 \pm 0.000$ & $0.109 \pm 0.000$ & $0.197 \pm 0.000$\\
			KDE & $0.362 \pm 0.000$ & $0.532 \pm 0.000$ & $0.333 \pm 0.000$ & $0.500 \pm 0.000$ & $0.240 \pm 0.000$ & $0.386 \pm 0.000$\\
			COBWEB & $0.277 \pm 0.000$ & $0.434 \pm 0.000$ & $0.334 \pm 0.000$ & $0.501 \pm 0.000$ & $0.196 \pm 0.000$ & $0.328 \pm 0.000$\\
			U-Net$_{traj}$ & $0.643 \pm 0.010$ & $0.783 \pm 0.007$ & $0.498 \pm 0.117$ & $0.657 \pm 0.109$ & $0.552 \pm 0.024$ & $0.711 \pm 0.020$\\
			\hline
			\multicolumn{7}{c}{\textbf{Aerial Image-based Approaches}}\\
			\hline
			%DeepRoadMapper & $0.668 \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.505 \pm 0.004$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.458 \pm 0.007$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
			%RoadTracer & $0.677 \pm 0.003$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.538 \pm 0.003$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.499 \pm 0.005$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
			%DeepRoadMapper-50-1e-3 & $0.636 \pm 0.010$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.469 \pm 0.034$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.406 \pm 0.032$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
			%RoadTracer-50-1e-3 & $0.627 \pm 0.029$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.495 \pm 0.044$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $0.448 \pm 0.033$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
			%DeepRoadMapper-50-1e-4 & $0.619 \pm 0.010$ & $0.765 \pm 0.008$ & $0.467 \pm 0.021$ & $0.636 \pm 0.020$ & $0.383 \pm 0.020$ & $0.553 \pm 0.020$\\
			%RoadTracer-50-1e-4 & $0.618 \pm 0.029$ & $0.764 \pm 0.023$ & $0.508 \pm 0.030$ & $0.674 \pm 0.026$ & $0.447 \pm 0.017$ & $0.617 \pm 0.017$\\
			DeepRoadMapper & $0.630 \pm 0.007$ & $0.773 \pm 0.005$ & $0.481 \pm 0.017$ & $0.650 \pm 0.016$ & $0.403 \pm 0.015$ & $0.575 \pm 0.015$\\
			RoadTracer & $0.658 \pm 0.012$ & $0.794 \pm 0.009$ & $0.512 \pm 0.023$ & $0.677 \pm 0.020$ & $0.475 \pm 0.013$ & $0.644 \pm 0.012$\\
			SegNet & $0.629 \pm 0.006$ & $0.772 \pm 0.005$ & $0.484 \pm 0.029$ & $0.652 \pm 0.026$ & $0.408 \pm 0.018$ & $0.578 \pm 0.018$\\
			DeconvNet & $0.589 \pm 0.010$ & $0.741 \pm 0.008$ & $ 0.450 \pm 0.011$ & $ 0.617 \pm 0.010$ & $0.265 \pm 0.022$ & $0.418 \pm 0.028$\\
			U-Net & $0.642 \pm 0.013$ & $0.782 \pm 0.010$ &  $0.479 \pm 0.024$ & $0.647 \pm 0.022$ & $0.409 \pm 0.019$ & $0.580 \pm 0.019$\\
			%FCN & $0.396 \pm 0.013$ & $0.567 \pm 0.014 $ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
			\hline
			\multicolumn{7}{c}{\textbf{Fusion-based Approaches}}\\
			\hline
			Early Fusion & $0.664 \pm 0.020$ & $0.798 \pm 0.015$ & $0.573 \pm 0.027$ & $0.728 \pm 0.021$ & $0.566 \pm 0.031$ & $0.723 \pm 0.025$\\
			Late Fusion & $0.674 \pm 0.005$ & $0.806 \pm 0.003$ & $0.553 \pm 0.027$ & $0.712 \pm 0.022$ & $0.561 \pm 0.027$ & $0.718 \pm 0.022$\\
			SegNet-RC (late fusion + correction) & $0.688 \pm 0.007$ & $0.815 \pm 0.005$ & $0.603 \pm 0.034$ & $0.752 \pm 0.027$ & $0.565 \pm 0.042$ & $0.721 \pm 0.035$\\
			FuseNet (encoder fusion) & $0.667 \pm 0.016$ & $0.800 \pm 0.011$ & $0.558 \pm 0.072$ & $0.714 \pm 0.062$ & $0.599 \pm 0.024$ & $0.749 \pm 0.019$\\
			V-FuseNet (encoder fusion) & $0.688 \pm 0.021$ & $0.815 \pm 0.015$ & $0.626 \pm 0.019$ & $0.770 \pm 0.015$ & $0.605 \pm 0.029$ & $0.754 \pm 0.023$\\
			L3Fsn & $0.675 \pm 0.003$ & $0.806 \pm 0.002$ & $0.603 \pm 0.012$ & $0.752 \pm 0.009$ & $0.555 \pm 0.032$ & $0.713 \pm 0.027$\\
			1D decoder & $0.664 \pm 0.037$ & $0.797 \pm 0.034$ & $0.610 \pm 0.018$ & $0.759 \pm 0.008$ & $0.599 \pm 0.016$ & $0.748 \pm 0.017$ \\
			TriSeg & $0.682 \pm 0.005$ & $0.811 \pm 0.004$ & $0.621 \pm 0.005$ & $0.767 \pm 0.004$ & $0.589 \pm 0.009$ & $0.742 \pm 0.007$\\
			\model & $\mathbf{0.717 \pm 0.003}$ & $\mathbf{0.835 \pm 0.002}$ & $\mathbf{0.634 \pm 0.012}$ & $\mathbf{0.776 \pm 0.009}$ & $\mathbf{0.620 \pm 0.025}$ & $\mathbf{0.765 \pm 0.019}$\\
			\hline
		\end{tabular}
	\end{center}    
	\vspace{-0.15in}
\end{table*}



%\begin{table}
%	\scriptsize
%	\vspace{-0.2in}
%	\caption{\label{tab:overall_eval} The performance of all approaches under three image-trajectory-paired datasets. TC1, KDE and COBWEB are not learning-based approaches thus their results are deterministic.}
%	\vspace{-0.1in}
%	\begin{center}
%		\begin{tabular}{c|ccc}
%			\hline
%			Dataset & \multicolumn{1}{c}{Porto} & \multicolumn{1}{c}{Shanghai} & \multicolumn{1}{c}{Singapore}\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Trajectory-based Approaches}}\\
%			\hline
%			TC1 & $0.153 \pm 0.000$ & $0.361 \pm 0.000$ & $0.109 \pm 0.000$ \\
%			KDE & $0.362 \pm 0.000$ & $0.333 \pm 0.000$ & $0.240 \pm 0.000$ \\
%			COBWEB & $0.277 \pm 0.000$ & $0.334 \pm 0.000$ & $0.196 \pm 0.000$ \\
%			U-Net$_{traj}$ & $0.643 \pm 0.010$ & $0.498 \pm 0.117$ & $0.552 \pm 0.024$\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Aerial Image-based Approaches}}\\
%			\hline
%			DeepRoadMapper & $0.630 \pm 0.007$ & $0.481 \pm 0.017$ & $0.403 \pm 0.015$\\
%			RoadTracer & $0.658 \pm 0.012$ & $0.512 \pm 0.023$ & $0.475 \pm 0.013$\\
%			SegNet & $0.629 \pm 0.006$ & $0.484 \pm 0.029$ & $0.408 \pm 0.018$\\
%			DeconvNet & $0.589 \pm 0.010$ & $ 0.450 \pm 0.011$ & $0.265 \pm 0.022$\\
%			U-Net & $0.642 \pm 0.013$ &  $0.479 \pm 0.024$ & $0.409 \pm 0.019$\\
%			%FCN & $0.396 \pm 0.013$ & $0.567 \pm 0.014 $ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Fusion-based Approaches}}\\
%			\hline
%			Early Fusion & $0.664 \pm 0.020$ & $0.573 \pm 0.027$& $0.566 \pm 0.031$\\
%			Late Fusion & $0.674 \pm 0.005$ & $0.553 \pm 0.027$& $0.561 \pm 0.027$\\
%			SegNet-RC  & $0.688 \pm 0.007$ & $0.603 \pm 0.034$ & $0.565 \pm 0.042$\\
%			FuseNet & $0.667 \pm 0.016$ & $0.558 \pm 0.072$ & $0.599 \pm 0.024$\\
%			V-FuseNet & $0.688 \pm 0.021$ & $0.626 \pm 0.019$ & $0.605 \pm 0.029$\\
%			L3Fsn & $0.675 \pm 0.003$ & $0.603 \pm 0.012$ & $0.555 \pm 0.032$\\
%			1D decoder & $0.664 \pm 0.037$ & $0.610 \pm 0.018$ & $0.599 \pm 0.016$ \\
%			TriSeg & $0.682 \pm 0.005$ & $0.621 \pm 0.005$ & $0.589 \pm 0.009$\\
%			\model & $\mathbf{0.717 \pm 0.003}$ & $\mathbf{0.634 \pm 0.012}$ & $\mathbf{0.620 \pm 0.025}$\\
%			\hline
%		\end{tabular}
%	\end{center}    
%	\vspace{-0.15in}
%\end{table}


%\begin{table}
%	\scriptsize
%	\vspace{-0.1in}
%	\caption{\label{tab:overall_eval} The IoUs of all approaches under three image-trajectory-paired datasets. TC1, KDE and COBWEB are not learning-based approaches thus their results are deterministic.}
%	\begin{center}
%		\begin{tabular}{c|ccc}
%			\hline
%			Dataset & \multicolumn{1}{c}{Porto} & \multicolumn{1}{c}{Shanghai} & \multicolumn{1}{c}{Singapore}\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Trajectory-based Approaches}}\\
%			\hline
%			TC1 & 0.153 $\pm$ 0.000 & 0.361 $\pm$ 0.000 & 0.109 $\pm$ 0.000 \\
%			KDE & 0.362 $\pm$ 0.000 & 0.333 $\pm$ 0.000 & 0.240 $\pm$ 0.000 \\
%			COBWEB & 0.277 $\pm$ 0.000 & 0.334 $\pm$ 0.000 & 0.196 $\pm$ 0.000 \\
%			U-Net$_{traj}$ & 0.643 $\pm$ 0.010 & 0.498 $\pm$ 0.117 & 0.552 $\pm$ 0.024\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Aerial Image-based Approaches}}\\
%			\hline
%			DeepRoadMapper & 0.630 $\pm$ 0.007 & 0.481 $\pm$ 0.017 & 0.403 $\pm$ 0.015\\
%			RoadTracer & 0.658 $\pm$ 0.012 & 0.512 $\pm$ 0.023 & 0.475 $\pm$ 0.013\\
%			SegNet & 0.629 $\pm$ 0.006 & 0.484 $\pm$ 0.029 & 0.408 $\pm$ 0.018\\
%			DeconvNet & 0.589 $\pm$ 0.010 & 0.450 $\pm$ 0.011 & 0.265 $\pm$ 0.022\\
%			U-Net & 0.642 $\pm$ 0.013 &  0.479 $\pm$ 0.024 & 0.409 $\pm$ 0.019\\
%			%FCN & $0.396 \pm 0.013$ & $0.567 \pm 0.014 $ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$ & $\textcolor{MyRed}{0.000} \pm 0.001$\\
%			\hline
%			\multicolumn{4}{c}{\textbf{Fusion-based Approaches}}\\
%			\hline
%			Early Fusion & 0.664 $\pm$ 0.020 & 0.573 $\pm$ 0.027 & 0.566 $\pm$ 0.031\\
%			Late Fusion & 0.674 $\pm$ 0.005 & 0.553 $\pm$ 0.027& 0.561 $\pm$ 0.027\\
%			SegNet-RC  & 0.688 $\pm$ 0.007 & 0.603 $\pm$ 0.034 & 0.565 $\pm$ 0.042\\
%			FuseNet & 0.667 $\pm$ 0.016 & 0.558 $\pm$ 0.072 & 0.599 $\pm$ 0.024\\
%			V-FuseNet & 0.688 $\pm$ 0.021 & 0.626 $\pm$ 0.019 & 0.605 $\pm$ 0.029\\
%			L3Fsn & 0.675 $\pm$ 0.003 & 0.603 $\pm$ 0.012 & 0.555 $\pm$ 0.032\\
%			1D decoder & 0.664 $\pm$ 0.037 & 0.610 $\pm$ 0.018 & 0.599 $\pm$ 0.016 \\
%			TriSeg & 0.682 $\pm$ 0.005 & 0.621 $\pm$ 0.005 & 0.589 $\pm$ 0.009\\
%			\model & \textbf{0.717} $\mathbf{\pm}$ \textbf{0.003} & \textbf{0.634} $\mathbf{\pm}$ \textbf{0.012} & \textbf{0.620} $\mathbf{\pm}$ \textbf{0.025}\\
%			\hline
%		\end{tabular}
%	\end{center}    
%	\vspace{-0.15in}
%\end{table}
